ScientoBASE: A Framework and Model for Computing Scholastic Indicators of non-local influence of Journals via Native Data Acquisition algorithms

Defining and measuring internationality as a function of influence diffusion of scientific journals is an open problem. There exists no metric to rank journals based on the extent or scale of internationality. Measuring internationality is qualitative, vague, open to interpretation and is limited by vested interests. With the tremendous increase in the number of journals in various fields and the unflinching desire of academics across the globe to publish in "international" journals, it has become an absolute necessity to evaluate, rank and categorize journals based on internationality. Authors, in the current work have defined internationality as a measure of influence that transcends across geographic boundaries. There are concerns raised by the authors about unethical practices reflected in the process of journal publication whereby scholarly influence of a select few are artificially boosted, primarily by resorting to editorial maneuvres. To counter the impact of such tactics, authors have come up with a new method that defines and measures internationality by eliminating such local effects when computing the influence of journals. A new metric, Non-Local Influence Quotient(NLIQ) is proposed as one such parameter for internationality computation along with another novel metric, Other-Citation Quotient as the complement of the ratio of self-citation and total citation. In addition, SNIP and International Collaboration Ratio are used as two other parameters.

==> referenc.tex <==

\begin{thebibliography}{99.}%
\bibitem{1}{}
G. Buchandiran, \emph{ An Exploratory Study of Indian Science and Technology
Publication Output},\hskip 1em plus 0.5em minus 0.4em\relax Department of
Library and Information Science, Loyola Institute of Technology Chennai
http://www.webpages.uidaho.edu/~mbolin/buchandiran.htm.

\bibitem{2}{}
Leonard Heilig and Stefan Voß, \emph{A Scientometric Analysis of Cloud
Computing Literature IEEE Transactions on Cloud Computing}, Vol. 2, No.
 3,\hskip 1em plus 0.5em minus 0.4em\relax July-September 2014

\bibitem {3}{}
Website : http://www.journalmetrics.com/values.php \emph{ As accessed on 6/3/2016.} 

\bibitem {4}{}
Website : http://www.journalindicators.com/methodology  \emph{ As accessed on 6/3/2016.} 

\bibitem {5}{}
Harzing, A.W. (2007) Publish or Perish, available from \emph{http://www.harzing.com/pop.htm} \emph{ As accessed on 6/3/2016.} 

\bibitem {6}{}
~Neelam Jangid, Snehanshu Saha, Anand Narasimhamurthy, Archana Mathur
\emph{Computing the Prestige of a journal: A Revised Multiple Linear Regression
Approach (2015)}; \hskip 1em plus
0.5em minus 0.4em\relax WCI- ACM Digital library(accepted), Aug 10-13, 2015.

\bibitem{7}{}
Neelam Jangid, Snehanshu Saha, Siddhant Gupta, Mukunda Rao J., \emph{Ranking of
Journals in Science and Technology Domain: A Novel And Computationally
Lightweight Approach}; \hskip1em plus
0.5em minus 0.4em\relax IERI Procedia, Elsevier, Vol 10(2014), pp 57–62;
doi:10.1016/j.ieri.2014.09.091

\bibitem{8}{}
Website:  http://www.scimagojr.com/journalrank.php   \emph{ As accessed on 6/3/2016.} 

\bibitem{9}{}
Seyyed Mehdi Hosseini Jenab, Ammar Nejati, \emph{Evaluation Of The Scientific
Production Of Countries By A Resource Scaled Two-Dimensional Approach};
\hskip1em plus
0.5em minus 0.4em\relax Journal of Scientometric Research, Sep–Dec 2014, Vol 3,
Issue 3.

\bibitem{10}{}
 Anup Kumar Das, Sanjaya Mishra, \emph{ Genesis Of Altmetrics Or Article-Level
 Metrics For Measuring Efficacy Of Scholarly Communications: Current
 Perspectives}, \hskip1em plus
0.5em minus 0.4em\relax Journal of Scientometric Research, May–Aug 2014, Vol 3,
Issue 2

\bibitem{11}{}
Gunther K. H. Zupanc, \emph{ Impact beyond the impact factor}, \hskip1em plus
0.5em minus 0.4em\relax J Comp Physiology A (2014) 200:113–116 Springer

\bibitem{12}{}
Ludo Waltman, Nees Jan van Eck, Thed N. van Leeuwen, Martijn S. Visser,
\emph{ Some modifications to the SNIP journal impact indicator},\hskip1em plus
0.5em minus 0.4em\relax Journal of Informetrics 7 (2013) 272– 285


\bibitem{13}{}
Gaby Haddow; Paul Genoni, \emph{ Citation Analysis And Peer Ranking Of
Australian Social Science Journals},\hskip1em plus 0.5em minus 0.4em\relax
Scientometrics, 85 (2) (2010) 471–487.

\bibitem{14}{}
Gualberto Buela-Casal, Pandelis Perkakis, Michael Taylor and Purificacion
Checha, \emph{ Measuring Internationality: Reflections And Perspectives On
Academic Journals}, \hskip1em plus
0.5em minus 0.4em\relax Scientometrics, 67 (1) (2006) 45-65.

\bibitem{15}{}
Chia-Lin Changa, Michael McAleer, Les Oxley, \emph {Coercive journal self
citations, impact factor, Journal Influence and Article Influence}, \hskip1em plus
0.5em minus 0.4em\relax Mathematics and Computers in Simulation 93 (2013) 190–197

\bibitem{16}{}
Abrizah; A.N. Zainab, K. Kiran, R.G. Raj \emph {LIS journals scientific impact
and subject categorization: a comparison between Web of Science and Scopus}, \hskip1em plus
0.5em minus 0.4em\relax Scientometrics (2013) 94:721–740 DOI 10.1007/s11192-012-0813-7

\bibitem{17}{}
Snehanshu Saha, Neelam Jangid, Archana Mathur, Anand M N \emph {DSRS: Estimation
and Forecasting of Journal Influence in the Science and Technology Domain via a
Lightweight Quantitative Approach}, \hskip1em plus
0.5em minus 0.4em\relax COLLNET Journal of  Scientometrics and Information
Management

\bibitem{18}{} 
http://www.crummy.com/software/BeautifulSoup/  \emph{ As accessed on 6/3/2016.} 

\bibitem{19}{}
http://scholarlyoa.com/publishers/  \emph{ As accessed on 6/3/2016.} 

\bibitem{20}{} 
https://en.wikipedia.org/wiki/Jeffrey\_Beall \emph{ As accessed on 6/3/2016.} 

\bibitem{21}{} 
 https://en.wikipedia.org/wiki/Predatory\_open\_access\_publishing   \emph{ As accessed on 6/3/2016.} 

\bibitem{22}{} 
 http://wokinfo.com/essays/impact-factor/

\bibitem{23}{} 
 Beall J. \emph {Predatory publishers are corrupting open access}, \hskip1em plus
 0.5em minus 0.4em\relax Nature. 2012;489:179

\bibitem{24}{}
Walt Crawford, (July 2014), \emph {"Journals, 'Journals' and Wannabes: Investigating The List"},\hskip1em plus
0.5em minus 0.4em\relax Cites \& Insights, 14:7, ISSN 1534-0937

\bibitem{25}{}
Jie Tang, Jing Zhang, Limin Yao, Juanzi Li, Li Zhang, and Zhong Su, \emph {ArnetMiner: Extraction and Mining of Academic Social Networks}, \hskip1em plus
0.5em minus 0.4em\relax Proceedings of the Fourteenth ACM SIGKDD International Conference on Knowledge Discovery and Data Mining (SIGKDD2008) pp.990-998

\bibitem{26}{} 
 https://aminer.org/billboard/citation  \emph{ As accessed on 21/1/2016.} 

 \bibitem{27}{}  
 https://www.youtube.com/watch?v=8IuQzq8fEYU \emph{ As accessed on 5/3/2016.}
 
 \bibitem{28}{}Snehanshu Saha, Neelam Jangid, Archana Mathur, Anand M N DSRS: \emph{ Estimation and Forecasting of Journal Influence in the Science and Technology , Domain via a Lightweight Quantitative Approach,} \hskip1em plus
0.5em minus 0.4em\relax COLLNET Journal of Scientometrics and Information Management; accepted in June 2016 Issue.

\bibitem{29}{}Henk F. Moed \emph{ Measuring contextual citation impact of scientific journals,} \hskip1em plus
0.5em minus 0.4em\relax Journal of Informetrics, Volume 4, Issue 3, July 2010

\bibitem{30}{} Snehanshu Saha, Avantika Dwivedi, Nandita Dwivedi, Gouri Ginde, Archana Mathur \emph{JIMI,Journal Internationality Modelling Index- An Analytical Investigation,} \hskip1em plus
0.5em minus 0.4em\relax Proceedings of the Fourth National Conference of Institute of Scientometrics, SIoT, August 2015

\bibitem{31}{} Gouri Ginde, Snehanshu Saha,
 Chitra Balasubramaniam, Harsha R.S,
 Archana Mathur, BS Dayasagar, Anand M N
\emph{Mining massive databases for computation of scholastic indices - Model and Quantify ‘internationality’ and ‘influence diffusion’ of peer-reviewed journals,} \hskip1em plus 0.5em minus 0.4em\relax Proceedings of the Fourth National Conference of Institute of Scientometrics, SIoT, August 2015

\bibitem{32}{} GitHub Repository for MATLAB code, information on JIMI - https://github.com/SciBase-Project/internationality-journals/blob/master/JIMI-JIS/ScientoBASE\_appendix.pdf \emph{ As accessed on 7/3/2016.}

\bibitem{34}{} Snehanshu Saha, Neelam Jangid, Archana Mathur, Anand M N
\emph{ DSRS: Estimation and Forecasting of Journal Influence in the Science and Technology Domain via a Lightweight Quantitative Approach} \hskip1em plus 0.5em minus 0.4em\relax 	arXiv:1604.03215

\bibitem{35}{Lutz Bornmann}
 http://arxiv.org/pdf/1407.2037.pdf

\bibitem{36}{2011}
Gingras, Y. (2014a). \emph{ The abuses of research evaluation, University World News. Retrieved} from http://www.universityworldnews.com/article.php?story=20140204141307557

\bibitem{37}{2014a}
 \emph{ How to boost your university up the rankings, University World News.
Retrieved} from  http://www.universityworldnews.com/article.php?story=20140715142345754

\bibitem{39}{2011}
Bhattacharjee, Y. (2011).  Saudi universities offer cash in exchange for academic prestige. Science, 334(6061), 1344-1345. doi:10.1126/science.334.6061.1344

\end{thebibliography}

